Evo-ViT: Slow-Fast Token Evolution for Dynamic Vision Transformer

Vision transformers (ViTs) have recently received explosive popularity, but the huge computational cost is still a severe issue. Since the computation complexity of ViT is quadratic with respect to the input sequence length, a mainstream paradigm for computation reduction is to reduce the number of tokens. Existing designs include structured spatial compression that uses a progressive shrinking pyramid to reduce the computations of large feature maps, and unstructured token pruning that dynamically drops redundant tokens. However, the limitation of existing token pruning lies in two folds: 1) the incomplete spatial structure caused by pruning is not compatible with structured spatial compression that is commonly used in modern deep-narrow transformers; 2) it usually requires a time-consuming pre-training procedure. To tackle the limitations and expand the applicable scenario of token pruning, we present Evo-ViT, a self-motivated slow-fast token evolution approach for vision transformers. Specifically, we conduct unstructured instance-wise token selection by taking advantage of the simple and effective global class attention that is native to vision transformers. Then, we propose to update the selected informative tokens and uninformative tokens with different computation paths, namely, slow-fast updating. Since slow-fast updating mechanism maintains the spatial structure and information flow, Evo-ViT can accelerate vanilla transformers of both flat and deep-narrow structures from the very beginning of the training process. Experimental results demonstrate that our method significantly reduces the computational cost of vision transformers while maintaining comparable performance on image classification.

==> Experiment_Outline.tex <==
Setting: 分类
Baseline: DeiT, LeViT
Dataset：ImageNet, Cifar10/100 (迁移)

方法：
1. pipline 总体方法介绍
2. token 选择
    基于class token attention的裁剪
    有放回：使得被裁掉token有后面被捡回来的机会
    global attention 稳定各层一致性
3. token更新
    additional token
4. 训练策略
    loss...
(5. 位置编码)

实验：
1. SOTA 方法对比


2. Ablation Study
    1. class token 作为裁剪策略的有效性 （对比其他可能的方法）
        (global) cls token
        (global) 列和
        spatial attention
    
    2. 方法各模块的有效性
        baseline (不裁剪)
        + 前一层prune
        + 有放回策略
        + global attention
        + update (additional token)
    
    3. 基于当前层裁剪 v.s. 基于前一层裁剪
        (可以说明基于前一层裁剪会更快)
        当前层
        前一层
        当前层 + global attention
        前一层 + global attention
        

    4. 超参数分析
        裁剪位置 (裁剪哪几层)
        裁剪比例
        更新global attention的trade-off
        (Position Embedding的维度)
    
    5. 可视化分析
        1. class token在各层高亮的规律 (放在第一页)
        
        2. prune结果可视化
        (对比各层裁剪的变化)    
            不裁剪
            + 单纯裁剪
            + Global Attention
            + Additional Token
    

    (6. Position Embedding的对比
        Ours
        PVT
        LeViT
        DeiT
    )    

==> Figs/fig_ablation.tex <==
\begin{figure*}[t]
\centering  %图片全局居中
\subfigure[]{
\label{fig:pruning_ratio_ablation}
\includegraphics[width=0.43\textwidth]{Imgs/pruning_ratio_ablation.pdf}}
\subfigure[]{
\label{fig:start_layer_ablation}
\includegraphics[width=0.43\textwidth]{Imgs/layer_ablation.pdf}}
\subfigure[]{
\label{fig:global_attn_tradeoff_ablation}
\includegraphics[width=0.43\textwidth]{Imgs/global_attn_tradeoff_ablation.pdf}}
\subfigure[]{
\label{fig:start_epoch}
\includegraphics[width=0.43\textwidth]{Imgs/acc-epoch.pdf}}
\caption{Ablation results on: (a) keeping ratio, (b) starting layer index, (c) global attention trade-off, (d) starting epoch.
% The corresponding definitions are described in the main text.
}
\label{fig:ablation}
\vspace{-4mm}
\end{figure*}

==> Figs/fig_ablation2.tex <==
\begin{figure}[t]
\centering  %图片全局居中
\subfigure[]{
\label{fig:pruning_ratio_ablation}
\includegraphics[width=0.22\textwidth]{Imgs/pruning_ratio_ablation.pdf}}
\subfigure[]{
\label{fig:start_layer_ablation}
\includegraphics[width=0.22\textwidth]{Imgs/layer_ablation.pdf}}
\caption{Ablation results on Hyper parameters: (a) keeping ratio, (b) starting layer index.
% The corresponding definitions are described in the main text.
}
\label{fig:ablation}
\end{figure}

==> Figs/fig_compare_curve.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{Imgs/compare_curve.png} % Reduce the figure size so that it is slightly narrower than the column.
\caption{SOTA comparision}
\label{fig:sota_curve}
\end{figure}

==> Figs/global_attn_tradeoff_ablation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{Imgs/global_attn_tradeoff_ablation.png} % Reduce the figure size so that it is slightly narrower than the column.
\caption{Global attention tradeoff ablation}
\label{fig:global_attn_tradeoff_ablation}
\end{figure}

==> Figs/pruning_ratio_ablation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{Imgs/pruning_ratio_ablation.png} % Reduce the figure size so that it is slightly narrower than the column.
\caption{Pruning ratio ablation}
\label{fig:pruning_ratio_ablation}
\end{figure}

==> Figs/start_layer_ablation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{Imgs/layer_ablation.png} % Reduce the figure size so that it is slightly narrower than the column.
\caption{Starting layer ablation}
\label{fig:start_layer_ablation}
\end{figure}

==> Figs/within_layer_correlation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{Imgs/within_layer_correlation.png}
    \caption{Token correlation coefficient}
    \label{fig:token_correlation}
\end{figure}

==> Sections/Experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Setup}
In this section, we demonstrate the superiority of the proposed Evo-ViT method through extensive experiments on the ImageNet-1k~\cite{imagenet} classification dataset. To demonstrate the generalization of our method, we conduct experiments on vision transformers of both flat and deep-narrow structures, \emph{i.e.}, DeiT~\cite{DeiT} and LeViT~\cite{LeViT}. For overall comparisons with the state-of-the-arts (SOTA) methods~\cite{DynamicViT,PatchSlimming,SViTE,IA-RED2}, we conduct the token selection and slow-fast token updating from the fifth layer of DeiT and 
the third layer (excluding the convolution layers) of LeViT, respectively. The selection ratio of informative tokens in all selected layers of both DeiT and LeViT are set to 0.5.
The global CLS attention trade-off $\alpha$ in Eqn.~\ref{eq:global_attn} are set to 0.5 for all layers.
For fair comparisons, all the models are trained for 300 epochs.

\subsection{Main Results}
\paragraph{Acceleration comparisons with state-of-the-art pruning methods.}
In Table~\ref{tab:prune_compare}, we compare our method with existing token pruning methods~\cite{DynamicViT,IA-RED2,PatchSlimming,SViTE}. Since token pruning methods are unable to recover the 2D structure and are usually designed for transformers with flat structures, we comprehensively conduct the comparisons based on DeiT~\cite{DeiT} on ImageNet dataset. We report the top-1 accuracy and throughput for performance evaluation. The throughput is measured on a single NVIDIA V100 GPU with batch size fixed to 256, which is same with the setting of DeiT. Results indicate that our method outperforms previous token pruning method on both accuracy and efficiency. Our method accelerate the inference at runtime by over 60$\%$ with negligible accuracy drop (-0.4$\%$) on DeiT-S.

\paragraph{Comparisons with state-of-the-art transformer models.}
Owing to the preserved placeholder tokens, our method guarantees the spatial structure that is indispensable for most existing modern vision transformer architectures.  Thus, we further apply our method to state-of-the-art efficient transformer LeViT~\cite{LeViT}, which presents a deep-narrow architecture. As shown in Table~\ref{tab:main_compare}, our method can further accelerate the deep-narrow transformer like LeViT in addition to remarkable performance on DeiT. 

\input{Tabs/comparision_prune_method}
\input{Tabs/main_exp}
\input{Tabs/method_ablation_deit}
\subsection{Ablation Analysis}
\paragraph{Effectiveness of each module.}
To evaluate the effectiveness of each sub-method, we add the following improvements step by step in Tab.~\ref{tab:method_ablation_deit} on both flat structure DeiT and deep-narrow structure LeViT:
\begin{itemize}
    \item Naive selection. Simply drop the uninformative tokens.
    \item Structural preservation. Preserve the uninformative tokens but not fast update them.
    \item Global attention. Utilize the proposed evolved global class attention instead of vanilla class attention for token selection.
    \item Fast updating. Augment the preserved placeholder tokens with fast updating.
    \item Layer to stage. Apply the proposed layer-to-stage training strategy to further accelerate inference.
\end{itemize}

Results on DeiT indicates that our structure preserving strategy can further improve the selection performance due to its capacity of preserving complete information flow. The global attention strategy enhances the consistency of token selection in each layer and achieves better performance. Fast updating strategy makes less effect on DeiT than on LeViT. We claim that the performance of DeiT turns to be saturated based on structure preservation and global attention while LeViT still has some space for improvement. LeViT exploits spatial pooling for token reduction, which makes unstructured token reduction in each stage more difficult. By using the fast updating strategy, it is possible to collect some extra cues from  placeholder tokens for accuracy and augment feature representations.
We also evaluate the layer to stage training strategy. Results indicate that it maintains the accuracy while further accelerating inference. 

\paragraph{Hyper parameter analysis.}
We further investigate the hyper parameters of our method on DeiT-T, namely, keeping ratio, starting layer index, global attention trade-off, and starting epoch. We initialize these hyper parameters as described in Setup. During ablation analysis, only the object parameter is changed and the others remain fixed. The layer-to-stage training strategy is disabled in the following ablation experiments.

\textit{Keeping ratio} determines how many tokens are kept for slow updating in each layer. For precision, we set all layers with the same keeping ratio and investigate the trade-off between accuracy and inference throughput in Fig.~\ref{fig:pruning_ratio_ablation}. Results show that the accuracy turns to be saturated when the keeping ratio is larger than 0.5. Another interesting finding is that the accelerated model with 0.9 keeping ratio outperforms the full baseline by 0.2$\%$ (72.2 to 72.4), which is consistent with the conclusion in \cite{SViTE} that properly dropping several uninformative tokens can serve as regularization for vision transformers.

\input{Figs/fig_ablation}
\input{Tabs/subsample_strategy_comparision}


\textit{Starting layer index} denotes which layer to start token selection and slow-fast updating. Fig.~\ref{fig:start_layer_ablation} indicates that the accuracy turns to be stable when we start from the fifth layer. We find a significant accuracy degradation as the starting layer becomes shallow, especially for the first three layers. We claim the reason lies that the features in these layers are still with large variation and not stable as shown in Fig.~\ref{fig:cka_score} and Fig.~\ref{fig:token_correlation}.

\textit{Global attention trade-off} in Eqn.~\ref{eq:global_attn} controls the dependence on previous layer information when conduct token selection in each layer. Larger trade-off leads to stronger dependence on previous information. Fig.~\ref{fig:global_attn_tradeoff_ablation} illustrates that it is the best to equally consider the previous and current information.

\textit{Starting epoch} denotes which epoch to start our token selection and updating strategy. As shown in Fig.~\ref{fig:start_epoch}, the accuracy drop sharply when we start from the last 100 epoch. We claim that the dynamic token selection requires enough training epochs to learn the refined features. For precision and training efficiency, we start our token selection and evolution strategy from the very beginning of training.


\paragraph{Different Token Selection Strategy.}
\input{Figs/different_ratio_ablation}
We further compare our global-attention-based token selection strategy with several common token selection strategies and subsampling methods in Tab.~\ref{tab:subsample_strategy_comparision} to evaluate the effectiveness of our method. All token selection strategies are conducted under our structure preserving strategy without layer-to-stage training schedule.

The token selection strategies include: randomly selecting the informative tokens (\textit{random selection}); Utilizing the class attention of the last layer for selection in all layers via two times inference (\textit{last class attention});  Utilizing the column mean of attention matrix to determine each token as proposed in~\cite{kim2021learned} (\textit{attention column mean}).

Results in Tab.~\ref{tab:subsample_strategy_comparision} indicate that our evolved global class attention outperform the other selection strategies and common subsampling methods on both accuracy and efficiency. We have observed an obvious performance degradation with last class attention, although the attention in deeper layers more focus on objects in Fig.~\ref{fig:fig1}. A possible reason lies that the networks require some background information to assist classification, while restricting all layers to only focus on objects during the entire training process leads to underfitting on the background features.

\paragraph{Visualization.}
\input{Figs/fig_prunevis}
We further visualize the token selection in Fig.~\ref{fig:prune_vis} to demonstrate performance of our method during both training and inference stages.  
The left three columns demonstrate results on different layers of a well-trained DeiT-T model. 
Results show that our token selection method mainly focuses on objects instead of backgrounds, thereby indicating that our method can effectively discriminate the informative tokens from placeholder tokens. 
The selection results tend to be consistent across layers, which proves the feasibility of our layer-to-stage training strategy.
Another interesting finding is that some missed tokens in the shallow layers are retrieved in the deep layers thanks to our structure preserving strategy.
Take the baseball images in the forth row as example, tokens of the bat are gradually picked up as the layer goes deeper.
We also investigate how the token selection evolves during the training stage in the right three columns. Results demonstrate that some informative tokens such as the fish tail are determined as placeholder tokens at the early epochs. With more training epochs, the ability of redundancy recognition of our method gradually increases and finally turns to be stable for discriminative token selection.

\paragraph{Consistent keeping ratio.} 
We set different keeping ratio in each layer to investigate the best accelerated architecture of Evo-ViT. Previous token pruning works~\cite{DynamicViT,PatchSlimming} present a staged architecture, in which more tokens are recognized as placeholder tokens in deeper layers. They are restricted in this type of architecture due to directly pruning. Our method allows more flexible token selection owing to the structure preserving slow-fast token evolution. As shown in Fig.~\ref{fig:abl_diff_pr}, we maintain the sum of the number of placeholder tokens in all layers and adjust the keeping ratio in each layer. Results demonstrate that the best performance is reached with a consistent keeping ratio across all layers. 
We explain the reason as follows. 
In the above visualization, we find that the selection results tend to be consistent across layers, indicating that the transformer tends to augment representations of meaningful informative tokens. 
In Fig.~\ref{fig:abl_diff_pr}, at most 50$\%$ tokens are passed through the full transformer network when the keeping ratios in all layers are set to $0.5$, thereby augmenting the most number of informative tokens with the best computing resources, namely, the full transformer network.

==> Sections/Experiments_v2.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Setup}
In this section, we demonstrate the superiority of the proposed Evo-ViT method through extensive experiments on the ImageNet-1k~\cite{imagenet} classification dataset. To demonstrate the generalization of our method, we conduct experiments on vision transformers of both flat and deep-narrow structures, \emph{i.e.}, DeiT~\cite{DeiT} and LeViT~\cite{LeViT}. For overall comparisons with the state-of-the-arts (SOTA) methods~\cite{DynamicViT,PatchSlimming,SViTE,IA-RED2}, we conduct the token selection and slow-fast token updating from the fifth layer of DeiT and 
the third layer (excluding the convolution layers) of LeViT, respectively. The selection ratio of informative tokens in all selected layers of both DeiT and LeViT are set to 0.5.
The global CLS attention trade-off $\alpha$ in Eqn.~\ref{eq:global_attn} are set to 0.5 for all layers.
For fair comparisons, all the models are trained for 300 epochs.

\subsection{Main Results}
\paragraph{Acceleration comparisons with state-of-the-art pruning methods.}
In Table~\ref{tab:prune_compare}, we compare our method with existing token pruning methods~\cite{DynamicViT,IA-RED2,PatchSlimming,SViTE}. Since token pruning methods are unable to recover the 2D structure and are usually designed for transformers with flat structures, we comprehensively conduct the comparisons based on DeiT~\cite{DeiT} on ImageNet dataset. We report the top-1 accuracy and throughput for performance evaluation. The throughput is measured on a single NVIDIA V100 GPU with batch size fixed to 256, which is same with the setting of DeiT. Results indicate that our method outperforms previous token pruning method on both accuracy and efficiency. Our method accelerate the inference at runtime by over 60$\%$ with negligible accuracy drop (-0.4$\%$) on DeiT-S.

\paragraph{Comparisons with state-of-the-art transformer models.}
Owing to the preserved placeholder tokens, our method guarantees the spatial structure that is indispensable for most existing modern vision transformer architectures.  Thus, we further apply our method to state-of-the-art efficient transformer LeViT~\cite{LeViT}, which presents a deep-narrow architecture. As shown in Table~\ref{tab:main_compare}, our method can further accelerate the deep-narrow transformer like LeViT in addition to remarkable performance on DeiT. 

\input{Tabs/comparision_prune_method}
\input{Tabs/main_exp}
\input{Figs/fig_prunevis}
\input{Tabs/method_ablation_deit}
\subsection{Ablation Analysis}
\paragraph{Effectiveness of each module.}
To evaluate the effectiveness of each sub-method, we add the following improvements step by step in Tab.~\ref{tab:method_ablation_deit} on both flat structure DeiT and deep-narrow structure LeViT:
\begin{itemize}
    \item Naive selection. Simply drop the uninformative tokens.
    \item Structural preservation. Preserve the uninformative tokens but not fast update them.
    \item Global attention. Utilize the proposed evolved global class attention instead of vanilla class attention for token selection.
    \item Fast updating. Augment the preserved placeholder tokens with fast updating.
    \item Layer to stage. Apply the proposed layer-to-stage training strategy to further accelerate inference.
\end{itemize}

Results on DeiT indicates that our structure preserving strategy can further improve the selection performance due to its capacity of preserving complete information flow. The global attention strategy enhances the consistency of token selection in each layer and achieves better performance. Fast updating strategy makes less effect on DeiT than on LeViT. We claim that the performance of DeiT turns to be saturated based on structure preservation and global attention while LeViT still has some space for improvement. LeViT exploits spatial pooling for token reduction, which makes unstructured token reduction in each stage more difficult. By using the fast updating strategy, it is possible to collect some extra cues from  placeholder tokens for accuracy and augment feature representations.
We also evaluate the layer to stage training strategy. Results indicate that it maintains the accuracy while further accelerating inference. 

% \paragraph{Hyper parameter analysis.}
% We further investigate the hyper parameters of our method on DeiT-T, namely, keeping ratio, starting layer index, global attention trade-off, and starting epoch. We initialize these hyper parameters as described in Setup. During ablation analysis, only the object parameter is changed and the others remain fixed. The layer-to-stage training strategy is disabled in the following ablation experiments.

% \textit{Keeping ratio} determines how many tokens are kept for slow updating in each layer. For precision, we set all layers with the same keeping ratio and investigate the trade-off between accuracy and inference throughput in Fig.~\ref{fig:pruning_ratio_ablation}. Results show that the accuracy turns to be saturated when the keeping ratio is larger than 0.5. Another interesting finding is that the accelerated model with 0.9 keeping ratio outperforms the full baseline by 0.2$\%$ (72.2 to 72.4), which is consistent with the conclusion in \cite{SViTE} that properly dropping several uninformative tokens can serve as regularization for vision transformers.

% \input{Figs/fig_ablation2}
% \input{Tabs/subsample_strategy_comparision}


% \textit{Starting layer index} denotes which layer to start token selection and slow-fast updating. Fig.~\ref{fig:start_layer_ablation} indicates that the accuracy turns to be stable when we start from the fifth layer. We find a significant accuracy degradation as the starting layer becomes shallow, especially for the first three layers. We claim the reason lies that the features in these layers are still with large variation and not stable as shown in Fig.~\ref{fig:cka_score} and Fig.~\ref{fig:token_correlation}.

% \textit{Global attention trade-off} in Eqn.~\ref{eq:global_attn} controls the dependence on previous layer information when conduct token selection in each layer. Larger trade-off leads to stronger dependence on previous information. Fig.~\ref{fig:global_attn_tradeoff_ablation} illustrates that it is the best to equally consider the previous and current information.

% \textit{Starting epoch} denotes which epoch to start our token selection and updating strategy. As shown in Fig.~\ref{fig:start_epoch}, the accuracy drop sharply when we start from the last 100 epoch. We claim that the dynamic token selection requires enough training epochs to learn the refined features. For precision and training efficiency, we start our token selection and evolution strategy from the very beginning of training.


% \paragraph{Different Token Selection Strategy.}
\input{Figs/different_ratio_ablation}
% We further compare our global-attention-based token selection strategy with several common token selection strategies and subsampling methods in Tab.~\ref{tab:subsample_strategy_comparision} to evaluate the effectiveness of our method. All token selection strategies are conducted under our structure preserving strategy without layer-to-stage training schedule.

% The token selection strategies include: randomly selecting the informative tokens (\textit{random selection}); Utilizing the class attention of the last layer for selection in all layers via two times inference (\textit{last class attention});  Utilizing the column mean of attention matrix to determine each token as proposed in~\cite{kim2021learned} (\textit{attention column mean}).

% Results in Tab.~\ref{tab:subsample_strategy_comparision} indicate that our evolved global class attention outperform the other selection strategies and common subsampling methods on both accuracy and efficiency. We have observed an obvious performance degradation with last class attention, although the attention in deeper layers more focus on objects in Fig.~\ref{fig:fig1}. A possible reason lies that the networks require some background information to assist classification, while restricting all layers to only focus on objects during the entire training process leads to underfitting on the background features.

\paragraph{Visualization.}
We further visualize the token selection in Fig.~\ref{fig:prune_vis} to demonstrate performance of our method during both training and inference stages.  
The left three columns demonstrate results on different layers of a well-trained DeiT-T model. 
Results show that our token selection method mainly focuses on objects instead of backgrounds, thereby indicating that our method can effectively discriminate the informative tokens from placeholder tokens. 
The selection results tend to be consistent across layers, which proves the feasibility of our layer-to-stage training strategy.
Another interesting finding is that some missed tokens in the shallow layers are retrieved in the deep layers thanks to our structure preserving strategy.
Take the baseball images in the forth row as example, tokens of the bat are gradually picked up as the layer goes deeper.
We also investigate how the token selection evolves during the training stage in the right three columns. Results demonstrate that some informative tokens such as the fish tail are determined as placeholder tokens at the early epochs. With more training epochs, the ability of redundancy recognition of our method gradually increases and finally turns to be stable for discriminative token selection.

\paragraph{Consistent keeping ratio.} 
We set different keeping ratio in each layer to investigate the best accelerated architecture of Evo-ViT. Previous token pruning works~\cite{DynamicViT,PatchSlimming} present a staged architecture, in which more tokens are recognized as placeholder tokens in deeper layers. They are restricted in this type of architecture due to directly pruning. Our method allows more flexible token selection owing to the structure preserving slow-fast token evolution. As shown in Fig.~\ref{fig:abl_diff_pr}, we maintain the sum of the number of placeholder tokens in all layers and adjust the keeping ratio in each layer. Results demonstrate that the best performance is reached with a consistent keeping ratio across all layers. 
We explain the reason as follows. 
In the above visualization, we find that the selection results tend to be consistent across layers, indicating that the transformer tends to augment representations of meaningful informative tokens. 
In Fig.~\ref{fig:abl_diff_pr}, at most 50$\%$ tokens are passed through the full transformer network when the keeping ratios in all layers are set to $0.5$, thereby augmenting the most number of informative tokens with the best computing resources, namely, the full transformer network.

==> Sections/Introduction.tex <==
\section{Introduction}
% 套话， Transformer 目前的进展，背景介绍
% --> 不同于nlp,在cv中存在冗余性(引用证明)
% 目前针对冗余性的解决现状 --> 我们发现class token是可以一定程度上反应冗余性的 (可视化证明)
% 有可视化结果得出class token具备一些其他特性，由此我们希望利用这种特性来构造精简的全局关系
% 与以往方法的不同（在以往方法基础上的提升和改进） --> 我们提出了一种基于class token的token裁剪策略，使得模型关注于重要有用的token
% 同时不失一般性地，一个无监督的token同样奏效
% 实验效果: DeiT上基本不掉点提速50%，无需finetune。 train from scatch; levit

% Background and development
% Transformer在cv各个领域都有建树
% Transformer强大的原因：独特的attention机制可以获取全局信息，矩阵运算具有effiecency
% 目前cv中常见的作法：把图像分patch输入作为token
Recently, transformers, dominated in natural language processing, have show its strong power on various computer vision tasks such as image classification, object detection, instance segmentation and low-level generalization. 
The reason of introducing transformers into computer vision lies on its unique properties that convolution neural networks lack, such as the long-range representation brought by self-attention. Most existing vision transformers split images to several patches as a sequence of input tokens.

\davina{Recently, transformers, dominated in natural language processing (NLP), have show strong power on various computer vision tasks such as image classification, object detection, instance segmentation and low-level generalization. The reason of introducing transformers into computer vision lies on its unique properties that convolution neural networks (CNN) lack, especially the property of modeling long-range dependencies in the data. However, different from NLP tasks, where most tokens are important due to the explicit grammatical structure, the modeling of long-range dependencies among image tokens across layers of the transformer usually brings redundancy and computation inefficiency because of low frequency information in backgrounds. }

% 不同于nlp,在cv中存在冗余性(引用证明)
% 不同在什么地方：nlp中每个token有明确的意义，对结果都有影响，cv中的token有图像的先验，背景token占多数但用处并不大 -->更稀疏。引用？
% (cv token数量更多)
Different from natural language processing, where most tokens are important due to the explicit grammatical structure, computer vision  always show a property of sparse representation. For example, background tokens accounted for a large part of an image contribute little to the final result, which is even worse with dense inputs. 
% 目前针对冗余性的解决现状
% 直接利用cnn的不好之处：经过直接裁剪的特征无法直接与transformer自身特征适配，需要通过进一步自蒸馏finetune来适配特征.导致的问题：1. 输入更dense 时无法不裁剪直接训 2. 只能适用于直筒型

\davina{To address the inefficiency problem of modeling long-range dependencies in vision transformers, existing methods follow three mainstreams. The first is to improve the computation efficiency of the multi-head self-attention (MSA) module\cite{PVT, CvT}. They structurally reduce the number of tokens by applying local-wise linear projection or convolutional projection for key and value embeddings respectively, instead of the standard positional-wise linear projection in ViT. Although achieving locality prior and efficiency, this kind of under-sampling takes object and background equally, which is not discriminative enough. The number of queries does not decrease, which limits the acceleration ratio of network inference. The second paradigm is network pruning. (cite Patch slimming method) develops a top-down patch slimming approach that can identify and remove redundant patches in the pre-defined network. The whole pruning scheme for vision transformers is conducted layer-wisely under a careful control of the network error, which is of high accuracy but not flexible enough for network training. The pruning mask is fixed for all instances, which seems running counter to the property of dynamic relation modeling of vision transformers. The third paradigm is token sparsification.
DynamicViT explores an unstructured and data-dependent downsampling strategy based on pre-trained vision transformers. A binary decision mask is learnt by conducting linear projections on token representations to abandon tokens of less importance in the inference stage. However, this kind of unstructured sparsification method is hard to be applied to vision transformers of the deep-narrow structure, which affects its extensibility to downstream tasks.}

\davina{In this paper, we denote the less informative tokens in the input instance as Placeholder Tokens. We claim that now that transformers have insight into global relationships among image tokens and learn for classification, itself is able to distinguish discriminative tokens from placeholder tokens for each instance. Moreover, considering the special architecture of transformers, we find that token pruning is not an inevitable way for efficiency design. By preserving placeholder tokens, and updating discriminative tokens and placeholer tokens differently in an efficient way, same acceleration can be achieved while the structures of transformers are preserved. Thus, the acceleration method is versatile for transformers of either straight-forward structure or deep-narrow structure as shown in fig1(a), and is friendly for downstream tasks. Meanwhile, placeholder tokens ensure complete information flow, which makes end-to-end training from scratch possible.}


To address the redundancy of tokens in visual transformers, several works introduce the effective methods on convolutional networks to transformers. Tang (Patch Slimming) proposes a token pruning method with all instance sharing the same set of tokens. Inspired by xxx (prune in cnn), Rao (DynamicVit) proposes a mask to learn the importance of each token and drop the less important tokens according to the learned mask in a instance level way. These methods all need an unprocessed pre-trained model to conduct self-distillation fine-tune, which makes these methods struggled in dense inputs and spacial sub-sampling (\textcolor{red}{need more details?}). 

% 我们希望利用transformer自身的性质设计策略。我们发现class token是可以一定程度上反应冗余性的 (可视化证明)
% 有可视化结果得出class token具备一些其他特性，由此我们希望利用这种特性来构造精简的全局关系


Differently, we hope to utilize the transformer-own properties to design our strategy and address the above drawbacks. By analysing the attention scores of class tokens across different layers, we find that class tokens always focus on important tokens even without supervision (see figure x). Inspired by this, we can construct sparse global relationship among tokens.

% 我们提出了一种基于class token的token裁剪策略，使得模型关注于重要有用的token.
% 我们的方法包括 有放回策略 和global attention。
% 先主要介绍有放回策略
\davina{Therefore, we propose a dynamic token evolution method that  discriminatibe tokens and placeholder tokens into account, and accelerate versatile vision transformers. 
By taking close look at the property of a vision transformer, we observe that a transformer itself can identify unimformative long-term relationships for each instance. namely the cls token of a transformer estimates importance of each token, and augments discriminative tokens with higher attention. as shown in Fig.1(b) Thus, taking advantage of cls tokens, discriminative tokens and placeholer tokens are determined, and dynamic update strategy can be designed for model efficiency. Specifically,  the placeholder tokens are coarsely updated and added to the original ones by skip connection. To further ensure the stability and consistency of determination of two kinds of tokens, a global class attention update strategy is proposed.
We evaluated the effectiveness of our method on two kinds of baseline models, namely transformers of straight-forward structures such as DeiT and deep-narrow transformers like the state-of-the-art model LeViT on ImageNet dataset.  Results  demonstrate that by pruning 50\% tokens from the forth layers of DeiT leads to over 50\% improvement on throughput with almost no accuracy drop.}

In this work, we propose a novel dynamic token slimming method with bootstrap updating that utilize the properties of class tokens, dubbed as xxxx. In particular, the class score of each tokens is set to determine which tokens to be pruned in a dynamic way. Instead of directly abandoned, in bootstrap updating, the dropped tokens are coarsely updated and added to the original ones by skip connection, which is like bootstrap sampling. The advantages of bootstrap updating lies on two points: 1) the mis-dropped token by the earlier layers may be picked up by the later layers; 2) the spacial structure that indispensable for most models with sub-sampling are maintained after token slimming.

% 介绍global attention
% 为了各层一致性，我们进一步提出global class attention 作为裁剪的指标 
% global attention 首次被xxx提出，我们与其不同在：我们是将其作为裁剪的标准，xxxxx. 怎么说好呢？
% 具体描述
To further enhance the consistancy of dropped tokens of different layers, we propose a global class attention as the base of token selection. The idea of global attention is first proposed in xxx to improve the skip connection in transformers. Differently, we \textcolor{blue}{xxxxxx}. Specifically, the class attention of each layers are added to a global attention. While token selecting, the global attention score of each tokens is used to judge which token to be pruned. 

% 我们的其他优势：更灵活，layer-wise；train from scatch

% 实验效果: DeiT上基本不掉点提速50%，无需finetune。 train from scatch; levit
We evaluated the effectiveness of our method on both baseline model DeiT and state-of-the-art model with sub-sampling LeViT on ImageNet dataset.  Results  demonstrate that by pruning 50\% tokens from the forth layers of DeiT leads to over 50\% improvement on throughput with almost no accuracy drop.





==> Sections/Methodology.tex <==
\section{Methodology}
\label{sec:methodlogy}
% token selection
%       class attention
%       placeholder token
%       global attention
% token update
%       additional token
%       fast ffn

% 总述：
% A closer look at class token attention: 发现其具有判别信息强弱token的能力
% Dynamic token selection based on placeholder token --> global attn: 由于保持了空间结构，我们可以进一步利用跨层的先验来稳定裁剪
% fast-slow token update

\subsection{Overview}
\input{Figs/fig_method}
In this section, we first make some further analysis on the class token attention to show its ability of redundancy recognition. After taking the analysis results into consideration, we give introduction to our structure preserving token selection method and a global class attention is proposed to enhance the stability and efficiency. Then, fast-slow token updating strategy is introduced to equip the placeholder tokens with coarse updating. Finally, the training details such as loss and other training strategy are introduced. Algorithm x precisely illustrates our method. 

\subsection{A closer look at class token attention}
% 分析class attention关于冗余性的特性：可视化，CKA
% 目的是说明class token是具有分辨uninformational tokens 和 discrimined tokens的能力的
% 证明我们基于class token选择token是可靠的


\subsection{Structure preserving token selection}
% 描述如何通过class token attention 选择token
% 描述place holder token, 进一步说明可以使得误裁token捡回，并且适用于空间下采样
% global attention，替换某个公式的一环即可

Since the effectiveness of class token to redundancy recognition, a natural idea is to utilize class token attention to guide informative token selection. For easier understanding, we first introduce a naive token selection paradigm based on the original class token attention and our full method replaces the class token attention with a global class token attention for better stability. As shown in figure x, we propose a xxx block that equip an original transformer block with our token selection paradigm. For each xxx block, which has $N$ input patch tokens $x \in \mathbb{R}^{N \times C}$ and their corresponding class token attention $A = \{A_{i}\}_{1}^{N}$, we conduct the structure preserving token selection by the following steps. First, the informative tokens, whose corresponding class attention score are among the top $k$  of class token attention $A$, are selected to pass the full transformer blocks. 

$A_{k}=\arg \max_{A^{\prime} \in A, |A^{\prime}|=k} \sum_{a \in A^{\prime}} a$

$x_{inf}=\{t|t \in A_{k} \cap x\}$

$x_{inf}=MLP(MSA(x_{inf}))$

Then, the placeholder tokens, which denote the unselected tokens, are kept and coarsely updated by a fast scheme rather than being abandoned. 

$x_{ph}= x \setminus x_{inf}$

$x_{ph}=f(x_{ph})$

where $f$ denotes the fast updating function, which will be introduced in the next section.

Finally, both the informative tokens and placeholder tokens are concatenate again to maintain the original spacial structure.

$x=\{x_{inf}, x_{ph}\}$

Thanks to the placeholder tokens, the mis-dropped token by the earlier layers may be picked up by the later layers. Furthermore, placeholder tokens preserve the spacial structure of each layer output, which enable our token selection method suitable for models with spacial sub-sampling like max pooling or convolution.

\paragraph{Global class attention.} In order to take both informative and placeholder tokens into selection procedure, a natural idea is to calculate the class attention score of each token at the beginning of each xxx block. However, this leads into nonnegligible additional computational cost, which is inconsistent with the acceleration goal. Thus, we propose a global class attention as the selection metrics. As shown in figure x, the global class attention is initialized by the first class token attention. In each self-attention module, we only need to update the global score of selected informative tokens by adding their class attention scores to corresponding global ones. During the token selection, the informative tokens are selected by current global class attention, which avoids re-calculating the class attention. The mathematical explanation can be derived by simply replacing the xxx in equation xxx, as shown in xxx.

$A_{0}=attn_{0}$

$\hat{A}_{n}=\hat{A}_{n-1}+attn_{n}$

\subsection{Fast-slow token updating}
% additional token：fast updating
During token selection, we denote the unselected tokens with less information as placeholder tokens.  As shown in figure x, the placeholder tokens usually represent background. Though of less importance, placeholder tokens are sometimes beneficial to the final results due to their causal relationship to informative tokens of main objects. For example, swimsuits (need substituted) are always of higher probability than dresses with ocean backgrounds. Thus, instead of being simply kept, placeholder tokens can bring more power with some fast and coarse updating. In xxx, we propose a novel fast-slow token updating strategy to equip the unselected placeholder tokens with an additional fast updating.

As shown in figure x, we integrate the placeholder tokens into a representative token by an aggregate function such as a transposed linear function or average pooling. Here we use a transposed linear
function in our method. Then, the generated representative token is combined with the selected informative tokens to go through the full MSA and FFN updating. Finally, the updated representative token is added back to the placeholder tokens by skip connection.

By representative tokens, the placeholder tokens are updated with negligible additional time cost. 


\subsection{Implementation Details}
% \subsection{Training and inference}
% layer-stage：稳定加速
% Avg pool + cls token 训练时加监督
% 强调train from scratch

% 为什么能train from scratch?

\paragraph{Layer-to-stage training schedule}

\paragraph{Assisted class token loss}

\paragraph{Complexity Analysis}
\begin{equation*}
    \begin{split}
        \mathcal{O}(SA) &= 4HWC^2 + 2(HW)^2C, \\
        \mathcal{O}(Ours) &= xxx.
    \end{split}
\end{equation*}

==> Sections/Related_Works.tex <==
\section{Related Work}
\paragraph{Vision Transformer}
Recently, a series of transformer models \cite{survey1,survey2,survey3} are proposed to solve various computer vision tasks. Transformer has achieved promising success in image classification \cite{ViT, DeiT, ConViT}, object detection \cite{DETR,shuffletransformer,SwinT,deformableDETR} and segmentation \cite{sstvos,SETR} due to its significant modeling capabilities of long-range dependencies. 

The pioneering works \cite{ViT,DeiT,LVViT} directly split an image into patches with fixed length and transform these image patches into tokens as inputs to a flat transformer. Vision Transformer (ViT) \cite{ViT} is one of such attempts that achieved state-of-the-art performance with large-scale pre-training. DeiT \cite{DeiT} manages to tackle the data-inefficiency problem in ViT by simply adjusting training strategies and adding an additional token along with the class token for knowledge distillation. 
To achieve better accuracy-speed trade-offs for general dense prediction, recent works~\cite{T2T,PiT,LeViT,PVT} design transformers of deep-narrow structures by adopting sub-sample operation (\emph{e.g.}, strided down sampling, local average pooling, convolutional sampling) to reduce the number of tokens in intermediate layers.
%Vision Transformer (ViT) \cite{} is the first work to design pure transformer for image classification on large-scale datasets.
% Besides, it prepends a learnable class token to the sequence of embeddings to integrate global information. 
%On the basis of ViT, DeiT \cite{} proposes an efficient distillation strategy and many training tricks to alleviate the need for large amounts of data in transformer. However, In the case of intensive input, this kind of methods will introduce redundant background tokens as described in Section \ref{sec:introduction} and take high computational cost.
%Therefore, large amount of methods \cite{T2T,PiT,LeViT} adopt sub-sample operation(\emph{e.g.}, strided down sampling, local average pooling, convolutional sampling) to reduce the number of tokens in intermediate layers and propose a deep narrow (\emph{i.e.}, simultaneously reduce token numbers and increase token dimension as the layer gets deeper) architecture for the balance of accuracy and efficiency. 
%For example, PiT \cite{PiT}  adopts depth-wise convolutions to decrease  the spatial resolution of features as most convolutional networks do.  LeViT \cite{LeViT} carefully designs a deep-narrow architecture and uses strided down sampling to reduce the number of tokens. \cite{CeiT} improve both the performance and the convergence speed of vision transformers by replacing the linear patch projection with convolutional layers and max-pooling, as well as modifying the feed-forward networks in each transformer layer to incorporate depth-wise convolutions.
%These structural sub-sample operations usually help reduce spatial redundancies among neighboring tokens and introduce some locality prior. Upon this kind of deep-narrow transformers, we claim that by preserving placeholder tokens and updating them in a slow way, unstructural redundancies can be further reduced and pyramid-like transformers can be equally accelerated as flat transformers.
These structural sub-sample operations usually help reduce spatial redundancies among neighboring tokens and introduce some locality prior. In this paper, we propose to handle instance-wise unstructured redundancies for both flat and deep-narrow transformers.



%Nevertheless, there exists considerable of less informative tokens in these models due to its hand-crafted architecture and structural sub-sample operation.
%In contrast, in this paper, we propose to preserve placeholder tokens and update discriminative tokens based on a simple token selection method to improve model efficiency.


% \vspace{-3mm}
\paragraph{Redundancy Reduction}
Transformer takes high computational cost because Multi-head Self-Attention (MSA) requires quadratic space and time complexity and Feed Forward Network (FFN) increases the dimension of latent features. The existing acceleration methods for transformers can be mainly categorized into sparse attention mechanism (\emph{e.g.}, low rank factorization \cite{CoaT,Linformer}, fixed local patterns and learnable patterns \cite{Synthesizer,longformer,SwinT}), pruning \cite{PatchSlimming,DynamicViT,LTH,PruningNIPS}, knowledge distillation \cite{distilbert} and so on. For example, \cite{SwinT} propose a shifted windowing scheme that brings greater efficiency by limiting self-attention computation to non-overlapping local windows while also allowing for cross-window connection.  The Linformer \cite{Linformer} is a classic example of low rank methods as it projects the length dimension of keys and values to a lower-dimensional representation. \cite{PatchSlimming} present a top-down layer-by-layer patch slimming algorithm to reduce the computational cost in pre-trained vision transformers. The patch slimming scheme is conducted under a careful control of the feature reconstruction error, so that the pruned transformer network can maintain the original performance with lower computational cost. \cite{DynamicViT} devise a lightweight prediction module to estimate the importance score of each token given the current features of a pre-trained transformer. The module is added to different layers to prune redundant tokens unstructurally and is supervised by a distillation loss based on the predictions of the original pre-trained transformer. In this paper, we propose to handle the redundancy problem from the very beginning of the training process of a versatile transformer. 

%fixed patterns methods \cite{} limit the calculation of attention to a fixed local pattern (\emph{e.g.}, block-wise pattern, strided pattern, compressed pattern) for reducing computational overhead while learnable pattern methods \cite{} introduce learnable hyper-parameters to split the entire sequence into subsequences and degrades the calculation of global attention into the calculation of local attention.

%Besides, many low rank methods \cite{} project keys and values into lower-dimensional representation and simultaneously approximates the multiplied matrix to original singular matrix. Token slimming is to remove redundant tokens. DynamicViT xxx. Token Slimming xxx. In this paper, we follow the research line of token slimming and propose a novel and robust token selection strategy to facilitate the balance of accuracy and efficiency.

==> Tabs/method_ablation_levit.tex <==
\begin{table}[]
\centering
\caption{Method ablation LeViT.}
\label{tab:method_ablation_levit}
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{lcc}
\toprule
Model               & Top-1 Acc. (\%) & Throughput (img/s) \\
LeViT 128S          &     74.5        &    8755            \\
+ placeholder token &     72.1        &    9892            \\
+ global attention  &     72.5        &    9752            \\
+ fast updating     &     73.2        &    9340            \\
+ layer to stage    &     73.2        &    9866            \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tabs/results_sup.tex <==
\begin{table}[t]
    \centering
    \caption{More results of Evo-ViT with dense image resolution. $^{*}$ denotes that the image resolution is $384 \times 384$.}
    \label{tab:sup_dense}
    \small{
    % \setlength{\tabcolsep}{1.5mm}{
    \begin{tabular}{l|cccc}
    \toprule
    \multirow{2}{*}{Method} & Batch Size & Top-1 Acc. & \multicolumn{2}{c}{Throughput}\\
     &  & (\%) & (img/s) & (\%) \\
    \midrule
    \multicolumn{4}{c}{DeiT-S} \\
    \midrule
    Baseline$^{*}$  &   128     &   OOM     &             258            &       -         \\
    Baseline$^{*}$  &   64      &   82.0    &             258            &       -         \\
    \textbf{Evo-ViT$^{*}$}      &   128     &   82.0    &             421            &    63.1    \\
    \midrule
    \multicolumn{4}{c}{DeiT-B} \\
    \midrule
    Baseline$^{*}$      &   64   &   OOM       &                87        &       -         \\
    \textbf{Evo-ViT$^{*}$}   &   64   &  82.0       &                139        &      59.8     \\
    \bottomrule
    \end{tabular}
    % }
    }
    \vspace{-5mm}
\end{table}

==> draft.tex <==
% Abstract Ouline
% 要突出的点：
% structure preserving: 保持完整信息流和完整空间结构 -> 适用于结构化压缩的模型，train from scratch


% 1. 目前Transformer进展巨大，但是冗余性计算仍然是一大问题。
% 2. 对于这个问题，目前主流的思路有 结构化压缩，如目前大多数mordern transformer 的 deep narrow型结构，以及token pruning.
% 3. 但是，目前的token pruning无法适用于结构化压缩的模型，且都需要一个完整的pretrain模型，这极大的限制了其适用性。这是因为pruning会破坏完整的空间结构->compressed models 和 完整的信息流->train from scratch
% 4. 我们。。。。。

